Moving Frame Net: SE(3)-Equivariant Network for Volumes

Equivariance of neural networks to transformations helps to improve their performance and reduce generalization error in computer vision tasks, as they apply to datasets presenting symmetries (e.g. scalings, rotations, translations). The method of moving frames is classical for deriving operators invariant to the action of a Lie group in a manifold.Recently, a rotation and translation equivariant neural network for image data was proposed based on the moving frames approach. In this paper we significantly improve that approach by reducing the computation of moving frames to only one, at the input stage, instead of repeated computations at each layer. The equivariance of the resulting architecture is proved theoretically and we build a rotation and translation equivariant neural network to process volumes, i.e. signals on the 3D space. Our trained model overperforms the benchmarks in the medical volume classification of most of the tested datasets from MedMNIST3D.

==> architecture_se3movfr.tex <==
\begin{tikzpicture}[block/.style={rectangle, rounded corners, draw}, node distance=.3cm]
	\node[block] (input) {\scriptsize \begin{tabular}{c} input \\ $f:\Omega \to \R$ \end{tabular}};
	
    \node[block, below=.5cm of input, fill=white] (deriv0) {\scriptsize \begin{tabular}{c}  Gaussian $2$-jets \\ $f^{(2)}_{\sigma'}: \Omega \to \R^{\binom{5}{2}}$ \end{tabular}};	
    \node[block, right=.5cm of deriv0, fill=red!30, anchor=west] (movfr) {\scriptsize $P$};	
    
	% \node[block, right=.6cm of input] (fmaps0) {\scriptsize \rotatebox{270}{feature maps}};
	\node[block, right=.6cm of input, fill=green!60] (block0) {\scriptsize \rotatebox{270}{SE3MovFBlock}};
	
	\node[block, right=of block0, fill=green!60] (block1) {\scriptsize \rotatebox{270}{SE3MovFBlock}};
	
	\node[circle, draw, inner sep=1pt, right=of block1] (sum1) {\scriptsize $+$};		
	
	\node[block, right=of sum1, fill=green!60] (block2) {\scriptsize \rotatebox{270}{SE3MovFBlock}};
	
	\node[circle, draw, inner sep=1pt, right=of block2] (sum2) {\scriptsize $+$};		
	
	\node[block, right=of sum2, fill=green!60] (block3) {\scriptsize \rotatebox{270}{SE3MovFBlock}};
	
	\node[circle, draw, inner sep=1pt, right=of block3] (sum3) {\scriptsize $+$};		
	
	
	\node[right=of sum3] (etc) {\scriptsize $\cdots$};		
	
	\node[block, right=of etc, fill=green!60] (block4) {\scriptsize \rotatebox{270}{SE3MovFBlock}};
	
	\node[circle, draw, inner sep=1pt, right=of block4] (sum4) {\scriptsize $+$};		
	
	\node[block, right=of sum4, fill=cyan!60] (pool) {\scriptsize \rotatebox{270}{GlobalMaxPooling}};
	
	\node[circle, draw, inner sep=1pt, right=of pool] (output) {\scriptsize $u_{\text{out}}$};		
	
	\draw[->] (input) -- (deriv0);
	\draw[->] (input) -- (block0);
	\draw[->] (block0) -- (block1);
	\draw[->] (block1) -- (sum1);
	\draw[->] (sum1) -- (block2);
	\draw[->] (block2) -- (sum2);
	\draw[->] (sum2) -- (block3);
	\draw[->] (block3) -- (sum3);
	\draw[->] (sum3) -- (etc);
	\draw[->] (etc) -- (block4);
	\draw[->] (block4) -- (sum4);
	\draw[->] (sum4) -- (pool);
	\draw[->] (pool) -- (output);
	
	\draw[->] (deriv0) -- (movfr);
	% \draw[->, draw=red!50, thick] (movfr) -- ++(.6cm,0) |- (inv0.west);
	% \draw[->, draw=red!50, thick] (movfr) -- ++(2.4,0) |- (block1.west);
	\draw[->, draw=red!50, thick] (movfr.north) -| (block0.south);
	\draw[->, draw=red!50, thick] (movfr) -| (block1.south);
	% \draw[->, draw=red!50, thick] (movfr) -| node[below] {\tiny prolonged SE$(3)$ action} (block2.south);
	\draw[->, draw=red!50, thick] (movfr) -| (block2.south);
	\draw[->, draw=red!50, thick] (movfr) -| (block3.south);
	\draw[->, draw=red!50, thick] (movfr) -|  (block4.south);
	
	\draw[->] (block0.east) -- ++(0.1,0.) |- ++(0,1.4) |- ++(1.2, 0.) |- (sum1.north);
	\draw[->] (sum1.east) -- ++(0.1,0.) |- ++(0,1.4) |- ++(1.2, 0.) |- (sum2.north);
	\draw[->] (sum2.east) -- ++(0.1,0.) |- ++(0,1.4) |- ++(1.2, 0.) |- (sum3.north);
	\draw[->] (etc.east) -- ++(0.1,0.) |- ++(0,1.4) |- ++(1.2, 0.) |- (sum4.north);
\end{tikzpicture}

==> equivariance_example.tex <==
\begin{tikzpicture}
    \node (orig) {\includegraphics[width=.1\textwidth]{figures/equiv3d_orig.pdf}};
    \node[right=2cm of orig] (rot) {\includegraphics[width=.1\textwidth]{figures/equiv3d_rot.pdf}};
    \node[below=.5cm of orig] (net) {\includegraphics[width=.1\textwidth]{figures/equiv3d_net.pdf}};
    \node[right=2cm of net] (netrot) {\includegraphics[width=.1\textwidth]{figures/equiv3d_netrot.pdf}};
    
    \draw[->, thick] (orig) -- node[below] {\tiny rotate and translate} (rot);
    \draw[->, thick] (orig) -- node[right] {\tiny $\phi$} (net);
    \draw[->, thick] (net) -- node[above] {\tiny rotate and translate} (netrot);
    \draw[->, thick] (rot) -- node[left] {\tiny $\phi$} (netrot);
\end{tikzpicture}

==> figures/medmnist3d_legend.tex <==
\definecolor{orangered}{HTML}{FF4620}
\definecolor{darkblue}{HTML}{000087}
\begin{tikzpicture}
    \node (cnn) at (0,0) {CNN};
    \node[right=0.5 of cnn.east] (cnn_end) {};
    
    \node[right=1 of cnn.east] (cnn_aug) {CNN augmented};
    \node[right=0.5 of cnn_aug.east] (cnn_aug_end) {};
    
    \node[right=1 of cnn_aug.east] (se3movf)  {SE3MovFNet};
    \node[right=0.5 of se3movf.east] (se3movf_end) {};
    
    \node[right=1 of se3movf.east] (se3movf_aug) {SE3MovFNet aug.};
    \node[right=0.5 of se3movf_aug.east] (se3movf_aug_end) {};
    
    \draw[thick, draw=red] (cnn.east) edge (cnn_end.west); 
    \draw[dashed, thick, draw=orangered] (cnn_aug.east) edge (cnn_aug_end.west); 
    \draw[thick, draw=blue] (se3movf.east) edge (se3movf_end.west); 
    \draw[dashed, thick, draw=darkblue] (se3movf_aug.east) edge (se3movf_aug_end.west); 
\end{tikzpicture}

==> legend.tex <==
\definecolor{orangered}{HTML}{FF4620}
\definecolor{darkblue}{HTML}{000087}
\begin{tikzpicture}
    \node (cnn) at (0,0) {CNN};
    \node[right=0.5 of cnn.east] (cnn_end) {};
    
    \node[right=1 of cnn.east] (cnn_aug) {CNN augmented};
    \node[right=0.5 of cnn_aug.east] (cnn_aug_end) {};
    
    \node[right=1 of cnn_aug.east] (se3movf)  {SE3MovFNet};
    \node[right=0.5 of se3movf.east] (se3movf_end) {};
    
    \node[right=1 of se3movf.east] (se3movf_aug) {SE3MovFNet aug.};
    \node[right=0.5 of se3movf_aug.east] (se3movf_aug_end) {};
    
    \draw[thick, draw=red] (cnn.east) edge (cnn_end.west); 
    \draw[dashed, thick, draw=orangered] (cnn_aug.east) edge (cnn_aug_end.west); 
    \draw[thick, draw=blue] (se3movf.east) edge (se3movf_end.west); 
    \draw[dashed, thick, draw=darkblue] (se3movf_aug.east) edge (se3movf_aug_end.west); 
\end{tikzpicture}

==> se3movfr_block.tex <==
\begin{tikzpicture}[scale=.65, 
                    block/.style={rectangle, rounded corners, draw},
                    node distance=.3cm,
                    background rectangle/.style={fill=green!60, rounded corners, draw},
                    show background rectangle]
    \node[block, fill=white] (input) at (0,0) {\scriptsize \begin{tabular}{c} input feature maps \\ $f_l:\Omega \to \R^q$ \end{tabular}};	
    \node[block, below=1.2cm of input.west, fill=red!30, anchor=west] (movfr) {\scriptsize \begin{tabular}{c} moving frame \\ $P:\Omega \to SO(3)$ \end{tabular}};	
    
    \node[block, right=of input, fill=white] (deriv) {\scriptsize \begin{tabular}{c}  Gaussian $n$-jets \\ $f^{(n)}_{l, \sigma}: \Omega \to \R^{q \binom{n+3}{n}}$ \end{tabular}};	
    \node[block, right=of deriv, fill=white] (inv) {\scriptsize \begin{tabular}{c} invariants \\ $P \cdot f^{(n)}_{l, \sigma}: \Omega \to \R^{q \binom{n+3}{n}}$ \end{tabular}};	
    \node[block, right=2cm of inv, fill=white] (fmaps) {\scriptsize \begin{tabular}{c} output features maps \\ $f_{l+1}: \Omega \to \R^q$ \end{tabular}};	
    
    
    \draw[->] (input) -- (deriv);
    \draw[->] (deriv) -- node[above] (virtual) {} (inv);
    \draw[->] (inv) -- node[below, anchor=south] {\tiny voxelwise MLP} (fmaps);
    
    \draw[->, draw=red!30, thick] (movfr.east) -| node[below] {\tiny prolonged SE$(3)$ action}  (virtual);
    
\end{tikzpicture}
